A conditional one-output likelihood formulation for multitask Gaussian processes

Multitask Gaussian processes (MTGP) are the Gaussian process (GP) framework's solution for multioutput regression problems in which the $T$ elements of the regressors cannot be considered conditionally independent given the observations. Standard MTGP models assume that there exist both a multitask covariance matrix as a function of an intertask matrix, and a noise covariance matrix. These matrices need to be approximated by a low rank simplification of order $P$ in order to reduce the number of parameters to be learnt from $T^2$ to $TP$. Here we introduce a novel approach that simplifies the multitask learning by reducing it to a set of conditioned univariate GPs without the need for any low rank approximations, therefore completely eliminating the requirement to select an adequate value for hyperparameter $P$. At the same time, by extending this approach with both a hierarchical and an approximate model, the proposed extensions are capable of recovering the multitask covariance and noise matrices after learning only $2T$ parameters, avoiding the validation of any model hyperparameter and reducing the overall complexity of the model as well as the risk of overfitting. Experimental results over synthetic and real problems confirm the advantages of this inference approach in its ability to accurately recover the original noise and signal matrices, as well as the achieved performance improvement in comparison to other state of art MTGP approaches. We have also integrated the model with standard GP toolboxes, showing that it is computationally competitive with state of the art options.

==> sections/intro_NIPS.tex <==
Gaussian processes (GP) \cite{rasmussen2006} are considered state of the art in nonlinear regression since they are a natural way to implement a predictive posterior distribution that provides a target mean together with a relevant measure of uncertainty in the form of a covariance. While standard GPs were initially designed to handle single scalar outputs, it is becoming more and more common to have to face multi-task (MT) or multidimensional output problems. This can be found in many application examples, such as multilabel scene classification  \cite{boutell2004learning}, patient stratification \cite{wiens2016patient}, age estimation \cite{Zhang2010} and, particularly with multioutput GP models, in  sensor networks \cite{11} or multioutput  time-series analysis \cite{13}. In these cases, the use of adequate approaches which are able to model the relationships among the tasks can offer significant advantages \cite{adiyeke2020benefits}.

There is a plethora of methods in the state of the art that tackle different particularizations of this problem (see \cite{liu2018remarks} for a review). In this paper we focus on multitask Gaussian process (MTGP) learning problems or symmetric multioutput problems where the objective is to jointly and symmetrically learn a set of $T$ tasks from the same observations. In this case, the joint treatment of all the tasks allows us to obtain a covariance matrix that models the relationships among tasks. This in turn can be used to obtain a multitask predictive posterior distribution.

The general MTGP formulation proposed in \cite{Bonilla2008}, and reformulated as a linear model of coregionalization (LMC) \cite{schmidt2003Bayesian, fanshawe2012bivariate}, assumes that the MT covariance matrix is expressed as the Kroneker product of an inter-task matrix $\bC$ and the input kernel matrix. 
Specifying a full rank $\bC$ requires a computational cost of $\mathcal{O}(N^3T^3)$ and the inference of $T(T- 1)/2$  parameters, which becomes computationally unwieldy when $T$ is large. In order to circumvent these problems, in \cite{Bonilla2008} authors use a low-rank approximation of order $P$ of $\bC$, $\bC\approx \bU \bLambda \bU^\top+\sigma^2\bI$, so that the number of parameters to be learnt is reduced from $\mathcal{O}(T^2)$ to $\mathcal{O}(TP)$ and the computational burden of the method is reduced from $\mathcal{O}(N^3T^3)$ to $\mathcal{O}(N^3T^2P)$. Parameter $P$ must be cross validated in order to obtain matrices that are representative of the process to be modelled, but authors usually choose a low value for parameter $P$ in order to keep the model's complexity low. In the particular case where $P=1$, this model simplifies into the well-known intrinsic coregionalization model (ICM) \cite{goovaerts1997geostatistics}, which allows significant computational savings. 

To obtain further computational savings in the general MTGP formulation, \cite{stegle2011efficient} proposes an efficient inversion of the MT covariance matrix by combining properties of the singular value decomposition (SVD) and the Kronecker product, reducing the computational cost from $\mathcal{O}(N^3T^2P)$ to $\mathcal{O}(N^3+T^3)$. These models consider a  noise model that is independent and identically distributed across tasks, i.e., their noise covariance matrices are of the form $\sigma^2\bI$. The approach in \cite{Rakitsch2013} offers a more general solution by introducing a noise covariance matrix which models inter-task noise dependencies. This results in a more realistic model with improved performance compared to the aforementioned alternatives. However, these methods have an important drawback in the number of parameters to be inferred. To mitigate this, the models presented in \cite{Bonilla2008, stegle2011efficient, Rakitsch2013} reduce the effective number of parameters of the inter-task covariance matrix by approximating it with a sum of $P$ rank one matrices that are further regularized in the GP model by the noise covariance term.

Additionally, several convolutional models \citep{lee2002, Boyle2005, Alvarez2008, alvarez2011computationally} have emerged, establishing a more sophisticated formulation that is able to model blurred relationships between tasks by the generalization of the MT kernel matrix through a convolution. However, adequate usage requires careful selection of the convolutional kernel in order to make the integral tractable, and the number of parameters must be limited to balance the model's flexibility against its complexity to avoid overfitting issues. Furthermore, this complex design limits the model's interpretability since the inter-task covariance matrices are not explicitly estimated. Efficient versions of these models \cite{alvarez2011computationally} introduce sparse GP formulations able to select $M$ inducing points to reduce the computational cost down to $\mathcal{O}(M^3T)$. 

%The usefulness of these multi-output Gaussian processes can be attested by the implementation of some of these models in into fully fledged libraries which are able to speed up training times. For example, we can find MTGP implementations in Pytorch \cite{GPTorch} or GPFlow \cite{GPflow2020multioutput}.


%Deep GP \cite{damianou2013} are networks inspired in deep belief networks where the layers are GP mappings. These models, trained using variational inference, are able to model multioutput GP through the use of different density models to the different outputs, all of them containing automatic relevance determination weights that have to be inferred. These models, nevertheless, do not provide with intertask covariance matrices.

Inspired by the MTGP probabilistic model proposed in \cite{Rakitsch2013}, where both the inter-task and noise covariance matrices are modelled, we introduce a novel learning methodology based on a decomposition of the likelihood function to turn the MT learning  process into a set of conditional one-output GPs. This methodology, combined with a hierarchical extension of the conditioned GPs, allows us to introduce the following novelties and advantages:
\begin{itemize}
\item[(1)] We do not need to use a low rank approximation of the inter-task covariance matrix, thus avoiding the selection of hyperparameter $P$.
\item[(2)] We reduce the number of parameters to be learnt in the noise and signal covariance matrices from $TP$ to $2T$, while recovering the full noise and intertask matrices. This reduces the model's complexity  and, as experiments show, leads to an improvement in performance.
%(3) This conditioned model, combined with an efficient implementation, leads to a computational time of $\mathcal{O}(N^3 + {T^4}/{4})$,  comparable to the one of \cite{stegle2011efficient,Rakitsch2013}  when $N>>T$. %; whereas the test computational time is $\mathcal{O}(N^3+T^3)$. 
\item[(3)] Finally, this learning approach can be easily adapted to leverage efficient GP libraries, such as Pytorch \cite{GPTorch}, allowing our method to be run on graphical processing units (GPU) with a computational burden of $\mathcal{O}(TN^2)$. In fact, this implementation is publicly available at \url{https://github.com/OGHinde/Cool_MTGP}. Additionally, in this case, the model also admits an embarrasingly parallel implementation over the tasks to get a computational cost per process of $\mathcal{O}({N^2})$.
\end{itemize}
%Besides, this inference can be parallelized over the tasks, with a computational cost per process of $\mathcal{O}({N^3})$, providing significant advantages if $T>N$. It can be easily adapted to be implemented with efficient GP library as Pytorch \cite{GPTorch} to be able to run over graphical processing units.%, or variational inducing variable implementations that use sparse matrices of $M<<N$ elements if a further computational cost reduction is needed. 

==> sections/intro_larga.tex <==

Gaussian processes (GP) \citep{rasmussen2006} can be considered state of the art in nonlinear regression, among other reasons, because they provide a natural way to implement a predictive posterior distribution. This distribution has a clear advantage over non-Bayesian models since  it is a surrogate statistical model that provides not only the predictive target means, but also a relevant measure of uncertainty in the form of a predictive covariance function.
%Gaussian process (GP) has been gaining widespread applications, e.g., small- or large-scale regression [4–6], dimensionality reduction [7], Bayesian optimization [8], uncertainty quantification [9] and time-series analysis [10].

While standard GPs were initially designed to handle single scalar outputs, it is becoming more and more common to have to face multi-task (MT) or multidimensional output problems in which each individual output cannot be considered conditionally independent from the rest given the predictors.

Typical GPs are usually designed for single-output scenarios. However, we frequently have to face multi-output problems where we are required to predict a set of tasks (a multidimensional output variable) which furthermore cannot be considered as conditionally independent given the predictors. This can be found in many application examples, such as multilabel scene classification  \cite{boutell2004learning}, patient stratification \cite{wiens2016patient}, age estimation \cite{Zhang2010} and, particularly with multioutput GP models, in  sensor networks \cite{11} or multioutput  time-series analysis \cite{13}. In these cases, the use of adequate approaches which are able to model the relationships among the tasks can offer significant advantages \cite{adiyeke2020benefits}.

%Examples of this can be found in  environmental sensor networks [11], robot inverse dynamics [12], multivariate physiological time-series analysis [13], structural design [14], aircraft design [15] and others.

%{\color{red} Falta introducir brevemente aquí los multi-task GPs para que el siguiente párrafo tenga sentido (o bien mover el siguiente párrafo más adelante).}

The usefulness of these multi-output Gaussian processes can be attested by the implementation of some of these models in into fully fledged libraries which are able to speed up training times. For example, we can find MTGP implementations in Pytorch \cite{GPTorch} or GPFlow \cite{GPflow2020multioutput}.




In these cases, we need particular approaches able to adequately model the relationships among the tasks and the intertask noise covariance. There is a plethora of methods in the state of the art that tackle different particularizations of this problem (see \cite{liu2018remarks} for a review). In this paper, we  focus on multitask Gaussian process (MTGP) learning problems or symmetric multioutput problems where the objective is to jointly and symmetrically learn a set of $T$ tasks from a single observation.  


%In \cite{liu2018remarks}, MTGP algorithms are classified in separable models, convolutional models and simple transformation models. 

Among all models, the MTGP proposed in \cite{Bonilla2008} can be considered the reference model, since other models as the one in  \cite{stegle2011efficient} and its generalization in  \cite{Rakitsch2013} are derived directly from it. That model assumes that a multitask covariance matrix exists which is expressed as the kroneker product of an intratask matrix $\bC$ and the input kernel matrix. Specifying a full rank $\bC$ requires a computational cost of $\mathcal{O}(N^3T^3)$ and the inference of $T(T- 1)/2$  parameters, which is unaffordable if $T$ is large. In order to circumvent these problems, in \cite{Bonilla2008} authors use a PCA or low-rank approximation of $\bC\approx \bU \bLambda \bU^\top+\sigma^2\bI$, where $\bU$ is a $T\times P$ matrix of the $P$ principal eigenvectors, which reduces the computational burden of the method to $\mathcal{O}(N^3T^2P)$ and number of parameters to be inferred to $\mathcal{O}(TP)$.  
This model can be reformulated as a linear model of coregionalization (LMC) (see e. g.  \cite{schmidt2003bayesian,fanshawe2012bivariate}), where the model outputs are expressed as a linear combination of $P$ latent functions and, therefore, the multitask kernel function can be also expressed as a linear combination of several covariance functions. 
Although authors usually choose a low value for parameter $P$ to reduce the model complexity, this parameter must be, in general, cross validated in order to obtain matrices that are representative of the process to be modelled. 

This model can be reformulated as a linear model of coregionalization (LMC) (see e. g.  \cite{schmidt2003bayesian,fanshawe2012bivariate}), where the model outputs are expressed as a linear combination of $P$ latent functions and, therefore, the multitask kernel function can be also expressed as a linear combination of several covariance functions. 

In the particular case where $P=1$, this model simplifies into the well-known intrinsic coregionalization model (ICM) [41] where this multitask covariance function is expressed as the kroneker product of an intratask matrix $C$ and the input kernel matrix, which allows significant computational savings. However, most of them have to introduce constraints in the matrix $C$ expression to reduce the number of parameters to be inferred when one is working with many task.

For instance, Osborne et al. [46] employed the ICM model and parametrized the correlation matrix as A = diag(e)STSdiag(e), where e corresponds to the length scale of each output and S is an upper triangular matrix describing the particular spherical coordinates of points. Besides, the semi- parametric latent factor model (SLFM) [47] defines the correlation matrix as Aq = aqaTq where aq = {at,q}1≤t≤T . In this case, Aq has a rank of one, and is equivalent to the free-form parameterization in what follows for P = 1.

In paper \cite{stegle2011efficient}, authors propose an efficient matrix inversion of the multitask covariance matrix  by combining the principal component analysis (PCA) of the mutlitask covariance matrix and the properties of the Kronecker product, reducing the computational cost to $O(N^3+T^3)$. These models consider a model that is independent and identically distributed across tasks, i.e., its matrix is $\sigma^2\bI$. The model in \cite{Rakitsch2013} generalizes the one in \cite{stegle2011efficient} by introducing a noise covariance matrix which model noise intertask dependencies. This approach leads to a more realistic model with improved performance  compared to the aforementioned alternatives.

These methods have an important drawback in the number of parameters to be inferred. The models presented in \cite{Bonilla2008,stegle2011efficient,Rakitsch2013} reduce the effective number of parameters of the intertask covariance matrices by approximating them with a sum of $P$ rank one matrices that are further regularized in the GP model by the noise covariance term. Authors choose a low value for parameter $P$, but it must be, in general, cross validated in order to obtain matrices that are representative of the process to be modelled. 
%that results in a total computational burden of $\mathcal{O}(N^3+T^3)$

On the other hand, we can also find in the literature the convolutional models \cite{lee2002,Boyle2005,Alvarez2008,alvarez2011computationally} which allow the modelling of blurred relationships between tasks by the generalization of the multitask kernel matrix through a convolution. The convolutional kernel has to be carefully selected in order to make the integral tractable. Also, the number of parameters must be limited in order to balance the model flexibility against its complexity in order to avoid  overfitting. Efficient versions of these models, such as the proposed of  \cite{alvarez2011computationally}, introduce sparse GP formulation to reduce the computational cost up to $O(M^3T)$, where $M$ is the number of inducing points.

Deep GP \cite{damianou2013} are networks inspired in deep belief networks where the layers are GP mappings. These models, trained using variational inference, are able to model multioutput GP through the use of different density models to the different outputs, all of them containing automatic relevance determination weights that have to be inferred. These models, nevertheless, do not provide with intertask covariance matrices.

In this paper a novel inference methodology for MTGP is introduced that solves the LMC problem in an efficient way. In particular, the problem is solved by using a factorization of the likelihood function by virtue of the chain rule of probability. This trick turns the multitask inference into a product of univariate conditional processes. This approach uses the same intertask and noise covariance matrices introduced in \cite{Rakitsch2013}, which are informative of the nature of the problem, and which is not provided by the convolutional models.  

The factorization trick used in our solution conveys a set of advantages with respect to previous models. The first one is that the complete intertask covariance and noise covariance matrices can be recovered from the conditional GPs parameters. So, the number of hyparameters to be inferred is $2T$ and low rank approximations are not needed, thus avoiding the cross validation of a low rank model. 

The computational burden of our method during the parameter inference or training is originally $\mathcal{O}(TN^3)$, but an efficient implementation  leads to a computational time of $\mathcal{O}(N^3 + \frac{T^4}{4})$. This computational time is comparable to the one of \cite{stegle2011efficient} and \cite{Rakitsch2013}  when $N>>T$. The computational time during the test phase is $\mathcal{O}(N^3+T^3)$. An additional advantage of the factorization trick relies in that our algorithm is highly parallelizable, with a computational cost per process of a single GP $\mathcal{O}{N^3}$, providing advantages if $T>N$. Finally, this model allows the use of any already implemented GP library as GPTorch, which runs over graphical processing units, or variational inducing variable implementations that use sparse matrices of $M<<N$ elements if a further computational cost reduction is needed. 


==> sections/intro_neurocomputing.tex <==
Gaussian processes (GP) \citep{rasmussen2006} can be considered state of the art in nonlinear regression, among other reasons, because they provide a natural way to implement a predictive posterior distribution. This distribution has a clear advantage over non-Bayesian models since  it is a surrogate statistical model that provides not only the predictive target means, but also a relevant measure of uncertainty in the form of a predictive covariance function. While standard GPs were initially designed to handle single scalar outputs, it is becoming more and more common to have to face multi-task (MT) or multidimensional output problems in which each individual output cannot be considered conditionally independent from the rest given the predictors. %This can be found in many application examples, such as multilabel scene classification  \cite{boutell2004learning}, patient stratification \cite{wiens2016patient}, age estimation \cite{Zhang2010} and, particularly with multioutput GP models, in  sensor networks \cite{11} or multioutput  time-series analysis \cite{13}. In these cases, the use of adequate approaches which are able to model the relationships among the tasks can offer significant advantages \cite{adiyeke2020benefits}.
 This can be found in many application examples, {\color{blue} such as medical applications \cite{wiens2016patient, BOUBNOVSKI2022}, air quality forecasting \cite{sun2021deep}, product design \cite{turetskyy2021} and, particularly with multioutput GP models, in multioutput time-series analysis \cite{13},  manufacturing applications \cite{Shen22}, detection of damages in structures \cite{LI2021110085}, forecast of multiscale solar radiation with application in photovoltaics  \cite{ZHOU2021124710}, or COVID-19 outbreak detection \cite{Ketu21}. See also the extensive survey on multi-output learning in \cite{Xu20}}. In these cases, the use of adequate approaches which are able to model the relationships among the tasks can offer significant advantages \cite{adiyeke2020benefits}.


%(2) Multitask classification, (3) multitask neural networks, (4) Neural networks, (5) Neural nets, lasso, others. (6) Bonilla (7) Bonilla con upper bounds (8) Bonilla (9) Bonilla (10) Bonilla


The general MTGP formulation proposed in \cite{Bonilla2008} can be considered the reference model and we will therefore refer to it in this paper as the standard MTGP (Std-MTGP). {\color{blue}Indeed, this model is the one chosen in all the above mentioned  MTGP applications}. This model assumes that the MT covariance matrix is expressed as the Kroneker product of an inter-task matrix $\bC$ and the input kernel matrix. Specifying a full rank $\bC$ requires a computational cost of $\mathcal{O}(N^3T^3)$ and the inference of $T(T- 1)/2$  parameters, which becomes computationally unwieldy when $T$ is large. In order to circumvent these problems, the authors of the Std-MTGP use a low-rank approximation of order $P$ of $\bC$, $\bC\approx \bU \bLambda \bU^\top+\sigma^2\bI$, so that the number of parameters to be learnt is reduced from $\mathcal{O}(T^2)$ to $\mathcal{O}(TP)$ and the computational burden of the method is reduced from $\mathcal{O}(N^3T^3)$ to $\mathcal{O}(N^3T^2P)$. This model is reformulated as a linear model of coregionalization (LMC) in \cite{schmidt2003Bayesian, fanshawe2012bivariate}, where the model outputs are expressed as a linear combination of $P$ latent functions and, therefore, the multitask kernel function can be also expressed as a linear combination of several covariance functions. In both cases, parameter $P$ must be cross validated in order to obtain matrices that are representative of the process to be modelled, but authors usually choose a low value for parameter $P$ in order to keep the model's complexity low. In the particular case where $P=1$, this model simplifies into the well-known intrinsic coregionalization model (ICM) \cite{goovaerts1997geostatistics}, which results in significant computational savings. To obtain further computational savings in the general MTGP formulation, \cite{stegle2011efficient} proposes an efficient inversion of the MT covariance matrix by combining properties of the singular value decomposition (SVD) and the Kronecker product, reducing the computational cost from $\mathcal{O}(N^3T^2P)$ to $\mathcal{O}(N^3+T^3)$. 


All the approaches cited so far consider a  noise model that is independent and identically distributed across tasks, i.e., their MT noise covariance matrices are of the form $\sigma^2\bI$. The approach in \cite{Rakitsch2013} offers a more general solution by introducing a noise covariance matrix which models inter-task noise dependencies. This results in a more realistic model with improved performance compared to the aforementioned alternatives. However, all of these methods have an important drawback in the number of parameters to be inferred. To mitigate this, the models presented in \cite{Bonilla2008, stegle2011efficient, Rakitsch2013} reduce the effective number of parameters of the inter-task covariance matrix by approximating it with a sum of $P$ rank one matrices that are further regularized in the GP model by the noise covariance term.

Additionally, several convolutional models \citep{lee2002, Boyle2005, Alvarez2008, alvarez2011computationally} have emerged, establishing a more sophisticated formulation that is able to model blurred relationships between tasks by the generalization of the MT kernel matrix through a convolution. However, adequate usage requires careful selection of the convolutional kernel in order to make the integral tractable, and the number of parameters must be limited to balance the model's flexibility against its complexity to avoid overfitting issues. Furthermore, this complex design limits the model's interpretability since the inter-task covariance matrices are not explicitly estimated. Efficient versions of these models \cite{alvarez2011computationally} introduce sparse GP formulations able to select $M$ inducing points to reduce the computational cost down to $\mathcal{O}(M^3T)$. 

{\color{blue} The main challenge for all these approaches (sse also \cite{chen2022multitask, NEURIPS2019_0118a063,nabati2022jgpr}),  lies in the fact that they have to fit a large number of parameters to model all the task relationships and, despite the fact that we can find many ad-hoc implementations that use very accurate optimizers \cite{GPTorch, DEWOLFF2021}, all these approaches are prone to fail in local minima, therefore resulting in suboptimal performance.}

{\color{blue}This work has been inspired by the MTGP probabilistic model featured in \cite{Rakitsch2013}, where the intertask and the noise covariances are explicitly modelled. Our proposal however presents a number of innovations and advantages that are summarized below. 

First, we rely on a new formulation based on a decomposition of the likelihood function into a set of conditional one-output GPs, combined with a hierarchical extension of the conditioned GPs. To our knowledge, this innovation has not been introduced before, and it leads to the following advantages. In the first place, as opposed to previous approaches, the one presented here does not need to use a low rank approximation of the inter-task covariance matrix. This avoids the need to select the corresponding hyperparameter (i.e: approximation rank parameter $P$ in \cite{Rakitsch2013} and others). 

This also means that the present methodology uses a full rank expression of the intertask covariance matrix, with $T(T-1)/2$ parameters. Despite this fact, the number of parameters to be learnt is reduced to $2T$, which is sufficient to recover the full noise and intertask covariance matrices, while previous approaches require $PT$ parameters to recover an intertask covariance of rank $P$.

The complexity of our model is also reduced, which leads to a reduction of the risk of overfitting and, hence, to an improvement in overall predictive performance.

Secondly, this learning approach can be easily adapted to leverage efficient GP libraries, such as Pytorch \cite{GPTorch} or MOGPTK \cite{DEWOLFF2021}, allowing our method to be run on graphical processing units (GPUs) with a computational burden of $\mathcal{O}(TN^2)$. In fact, this implementation is publicly available at \url{https://github.com/OGHinde/Cool_MTGP}. Additionally, in this case, the model also admits an embarrasingly parallel implementation over the tasks to get a computational cost per process of $\mathcal{O}({N^2})$.
}
